When is Task Vector Provably Effective for Model Editing? A Generalization Analysis of Nonlinear Transformers

Task arithmetic refers to editing the pre-trained model by adding a weighted sum of task vectors, each of which is the weight update from the pre-trained model to fine-tuned models for certain tasks. This approach recently gained attention as a computationally efficient inference method for model editing, e.g., multi-task learning, forgetting, and out-of-domain generalization capabilities. However, the theoretical understanding of why task vectors can execute various conceptual operations remains limited, due to the highly non-convexity of training Transformer-based models. To the best of our knowledge, this paper provides the first theoretical characterization of the generalization guarantees of task vector methods on nonlinear Transformers. We consider a conceptual learning setting, where each task is a binary classification problem based on a discriminative pattern. We theoretically prove the effectiveness of task addition in simultaneously learning a set of irrelevant or aligned tasks, as well as the success of task negation in unlearning one task from irrelevant or contradictory tasks. Moreover, we prove the proper selection of linear coefficients for task arithmetic to achieve guaranteed generalization to out-of-domain tasks. All of our theoretical results hold for both dense-weight parameters and their low-rank approximations. Although established in a conceptual setting, our theoretical findings were validated on a practical machine unlearning task using the large language model Phi-1.5 (1.3B).

==> problem_formulation.tex <==
\section{Problem Formulation}

Following \citep{IRWS22}, we study the performance of the model on different tasks by combining multiple task vectors together. Specifially, consider data $\bfX=(\bfx_1,\bfx_2,\cdots,\bfx_P)\in\mathbb{R}^{d\times P}$ that contains $P$ tokens, where each token is $d$-dimensional and  $\|\bfx_i\|=1$ for $i\in[P]$. The label $y\in\{+1,-1\}$ is a scalar. 

The \textbf{learning model} is a single-head one-layer Transformer with one self-attention layer and one two-layer perceptron, which is mathematically written as

\begin{equation}
    f(\bfX; \Psi)=\frac{1}{P}\sum_{l=1}^P\bfa_{(l)}^\top\text{Relu}(\bfW_O\bfW_V\bfX^n\text{softmax}_l({\bfX}^\top\bfW_K^\top\bfW_Q\bfx_l)),\label{eqn: network raw}
\end{equation}

where $\Psi=\{\{\bfa_{(l)}\}_{l=1}^P, \bfW_O,\bfW_V,\bfW_K,\bfW_Q\}$ denotes the set of all the model parameters. $\bfa_{(l)}\in\mathbb{R}^m$ and $\bfW_O\in\mathbb{R}^{m\times m_a}$ are weights in the MLP layer. $\bfW_V\in\mathbb{R}^{m_a\times d}$, $\bfW_K,\bfW_Q\in\mathbb{R}^{m_b\times d}$ are weights in the self-attention layer. $\text{softmax}_l((\bfW_K\bfx_i)^\top\bfW_Q\bfx_l)=e^{(\bfW_K\bfx_i)^\top\bfW_Q\bfx_l}/\sum_{j=1}^P e^{(\bfW_K\bfx_j)^\top\bfW_Q\bfx_l}$. $\min\{m_a, m_b\}>d$. 


Consider $\{\bfX^n, y^n\}_{n=1}^N$ as a dataset with $N$ data points for the task function $\mathcal{T}$, i.e., $y^n=\mathcal{T}(\bfX^n)$ for $n\in[N]$.  Each pair of $(\bfX^n, y^n)$ follows an unknown distribution $\mathcal{D}_\mathcal{T}$. Given a pre-trained model $\Psi^{(0)}$, we fine-tune the model by minimizing the empirical risk function to obtain the \textbf{task vector} $\Delta \Psi_\mathcal{T}$ for $\mathcal{T}$,
\begin{equation}
\begin{aligned}
    \Delta\Psi_\mathcal{T}=\Psi_\mathcal{T}^*-\Psi^{(0)}, \text{ where }
    \Psi_\mathcal{T}^*=\arg\min_{\Psi} \frac{1}{N}\sum_{n=1}^N \ell(\bfX^n,y^n;\Psi),
\end{aligned}
\end{equation}
and $\ell(\bfX,y; \Psi)$ is the loss function of $(\bfX,y)$ with the model $\Psi$. We use the Hinge loss $\ell(\bfX,y,\Psi)=\max\{1-y\cdot f(\bfX;\Psi),0\}$ as the loss function, where $f(\bfX;\Psi)$ is defined as in (\ref{eqn: network raw}). 

\iffalse
\textbf{Generalization with task vectors} Given the pre-trained model $\Psi^{(0)}$ and a set of task vectors $\{\Delta\Psi_{\mathcal{T}_i}\}_{i\in\mathcal{V}}$, we define the \textbf{generalization error} on the data $(\bfX,y)\sim\mathcal{D}_{\mathcal{T}'}$ for the task $\mathcal{T}'$ with the model $\Psi=\Psi^{(0)}+\sum_{i\in\mathcal{V}}\lambda_i\Delta\Psi_{\mathcal{T}_i}$, $\lambda_i\in\mathbb{R}$, as
\begin{equation}
    \mathbb{E}_{(\bfX,y)\sim\mathcal{D}_{\mathcal{T}'}}\ell(\bfX,y;\Psi).
\end{equation}
\fi


\textbf{Fine-tuning Algorithm for task vectors} For simplicity of analysis, we let $\bfW=\bfW_K^\top\bfW_Q\in\mathbb{R}^{d\times d}$ and $\bfV=\bfW_O\bfW_V\in\mathbb{R}^{m \times d}$ as \citep{JSL22, HCL23, ZFB23, HWCL24}. We use stochastic gradient descent (SGD) to fine-tune the model. At the $t$-th iteration, $t=0,1,\cdots,T-1$, the gradient is computed using a mini-batch $\mathcal{B}_t$ with $\mathcal{B}_t=B$. The step size is $\eta\leq O(1)$. Every entry of $\bfW$ and $\bfV$ is initialized from $\mathcal{N}(0,\xi^2)$ where $\xi\leq 1/\sqrt{m}$. Each $a_i$ is sampled from $\{+1/m, -1/m\}$. $a_{(l)}$ does not update during the fine-tuning.
